Improved Bilinear Pooling with CNNs

Bilinear pooling of Convolutional Neural Network (CNN) features [22, 23], and their compact variants [10], have been shown to be effective at fine-grained recognition, scene categorization, texture recognition, and visual question-answering tasks among others. The resulting representation captures second-order statistics of convolutional features in a translationally invariant manner. In this paper we investigate various ways of normalizing these statistics to improve their representation power. In particular we find that the matrix square-root normalization offers significant improvements and outperforms alternative schemes such as the matrix logarithm normalization when combined with elementwise square-root and l2 normalization. This improves the accuracy by 2-3% on a range of fine-grained recognition datasets leading to a new state of the art. We also investigate how the accuracy of matrix function computations effect network training and evaluation. In particular we compare against a technique for estimating matrix square-root gradients via solving a Lyapunov equation that is more numerically accurate than computing gradients via a Singular Value Decomposition (SVD). We find that while SVD gradients are numerically inaccurate the overall effect on the final accuracy is negligible once boundary cases are handled carefully. We present an alternative scheme for computing gradients that is faster and yet it offers improvements over the baseline model. Finally we show that the matrix square-root computed approximately using a few Newton iterations is just as accurate for the classification task but allows an order-of-magnitude faster GPU implementation compared to SVD decomposition.

==> matrix-sqrt.tex <==
Ionescu \etal~\cite{foo} explores matrix backpropagation and provides a fomula to compute the derivative of matrix square root  with respect to the input matrix. Given input matrix $X=U\Sigma U^T$, the matrix square root is expressed as $A=f(X)=Ug(\Sigma)U^T$, where $g$ takes square root on the diagonal entries. The function $L$ computes the loss based on the features $A$. The gradient of loss with respect to $X$ is obtained by chain rule as follow:
\begin{equation}
\frac{\partial L}{\partial X} = U\Bigg\{ \bigg( \tilde{K}^T \odot \bigg( U^T\frac{\partial L}{\partial U}\bigg) \bigg) + \bigg( \frac{\partial L}{\partial \Sigma}\bigg)_{diag}\Bigg\}U^T
\end{equation}
where $\odot$ denotes element-wise matrix multiplication. The derivatives of eigenvectors $\frac{\partial L}{\partial U}$ and eigenvalues $\frac{\partial L}{\partial \Sigma}$ are the derived as follow:

\begin{equation*}
\frac{\partial L}{\partial U} = \bigg\{ \frac{\partial L}{\partial A} + \bigg(\frac{\partial L}{\partial A}\bigg)^T\bigg\}Ug(\Sigma),
\quad
\frac{\partial L}{\partial \Sigma} = g'(\Sigma)U^T\frac{\partial L}{\partial A}U
\end{equation*}
The matrix $\tilde{K}^T$ defined as Equation~\ref{eqn:K} scales the gradients from eigenvectors by the difference between corresponding eigenvalues. This matrix potentially leads to numerical instability when (1) eigenvalues are small or (2) two eigenvectors have same eigenvalues. The small eigenvalues can be ignored by low-rank approximation of matirx. However, there is no simple way to avoid the second case.

\begin{equation}\label{eqn:K}
\tilde{K}_{i,j} = 
\begin{cases}
	\frac{1}{\sigma_i-\sigma_j}  & \quad \text{if } i\neq j\\
	0 & \quad \text{if } i=j\\
\end{cases}
\end{equation}
An alternative way to compute the derivatives of matrix square root is solving Lyapunov equation (Equation~\ref{eqn:lyap}).

\begin{equation}\label{eqn:lyap}
X\frac{\partial L}{\partial X} + \frac{\partial L}{\partial X}X^T = \frac{\partial L}{\partial A}
\end{equation}
The solution to the equation involves taking inverse of the square root of diagonal matrix $\Sigma$, so thus it does not suffer from the close eigenvalues and is more computationally stable.


